Interaction Techniques for Exploratory Data Visualization on Mobile Devices

The ubiquity and on-the-go availability of mobile devices makes them central to many tasks such as interpersonal communication and media consumption. However, despite the potential of mobile devices for on-demand exploratory data visualization, existing mobile interactions are difficult, often using highly custom interactions, complex gestures, or multi-modal input. We synthesize limitations from the literature and outline four motivating principles for improved mobile interaction: leverage ubiquitous modalities, prioritize discoverability, enable rapid in-context data exploration, and promote graceful recovery. We then contribute thirteen interaction candidates and conduct a formative study with twelve participants who experienced our interactions in a testbed prototype. Based on these interviews, we discuss design considerations and tradeoffs from four main themes: precise and rapid inspection, focused navigation, single-touch and fixed orientation interaction, and judicious use of motion.

==> icebox.tex <==
%!TEX root = proceedings.tex

\section{Icebox}


\noindent\jane{Interaction can have a broad definition, and one form of interaction we haven't discussed yet is \textbf{orientation} of the mobile device. We might think about responsive design as designing to encourage users to hold the device in a certain way for the best experience (for example, if I watch videos on my phone, I almost always do so in landscape orientation); this came to mind as an interesting design consideration for this project during a discussion this week (5/19)}

  Flexible and easy-to-use interactions for responsive visualization remains an open challenge due to the limited screen size and available modalities compared to desktop computers.
  In response, we summarize central concerns with interaction design on portable devices, and outline common issues with existing interactions.
%   In response, we contribute a novel interaction paradigm for responsive data visualization on mobile devices.
%   We introduce the concept of ``auto-complete'' interactions to efficiently disambiguate user intents, and provide a set of linear constraints over candidate transforms to minimize auto-completion errors.
  We present a novel interaction vocabulary rooted in simple touch and motion, covering an expressive gamut of visualization types and analysis tasks, and empirically refine our vocabulary through task-based \jane[discussions]{update terminology to be more concrete once methods are settled upon} with \luke{16} data analysts.
  We couple our interactions with modifications to the underlying visualization design, allowing users to engage with simple designs yet maintain flexibility in the analysis space. 
  We provide a two-part evaluation: (1)~a discussion of \todo{X} use cases in data analysis and journalism and (2)~a first-use study comparing our mobile interaction paradigm with traditional desktop interactions, \todo{finding that users preferred our simpler, more direct mobile interactions, despite faster completion time with desktop.}
  \\

\jane[Data visualizations typically use desktop peripheries and related WIMP (windows, icons, menus, pointer) metaphors for interactive analysis and exploration, despite broader use of mobile devices.]{Compared to the rest of the abstract, this sentence feels a bit out of place; the connection to the other parts of the abstract are not explicitly outlined and it leaves it up to the reader to reason about why this matters. In an attempt to do this, I've tried to distill the two main points that I see in this sentence: (1) while mobile devices are more often used for many other tasks, visualization is not one of them; (2) interaction is currently easier/more flexible on desktop, which is why that is the preferred place for analysis/exploration. I wonder if we could just start with the second sentence, as it makes the focus of this work and the challenges more clear; we could even try to add some of the other details into the sentence, e.g., Accessible, easy-to-use, and flexible interactions for mobile visualization analysis and exploration remains an open challenge due to the limited screen size and available modalities compared to desktop computers.}

\noindent\jane{Feel free to move any content that should be removed from the paper to this section (to keep individual section files clean). This section can act as an archive from which to restore content if we so choose. We can easily exclude this file from the final submission by commenting out or deleting the \texttt{\textbackslash input\{icebox\}} line from the end of the document.}

\noindent\luke{[Prior abstract] Interactive data visualizations are typically designed on desktop computers, although they are increasingly consumed on mobile devices. 
  This results in often ill-designed interactions that fail to enhance analysis with mobile-specific features.
  In response, we analyze a corpus of mobile visualizations to determine interaction deficiencies, and conduct formal interviews with  data analysts to outline improvements for mobile interaction. 
  Based on our interview findings, we present a new mobile interaction paradigm that optimistically predicts interaction intent based on touch gesture and view context. 
  To support mobile design, we incorporate our interaction paradigm in an authoring system that enables visualization developers to specify how users' view-contextualized gestures should adapt the visualization. 
  We evaluate with a first-use study to compare our mobile interaction paradigm to traditional desktop interactions, finding that users are able to generate insights more rapidly with our approach.}
  
  \noindent\luke{
    Approach:
    \begin{enumerate}
        \item Motivation with journalism examples (analysis examples more difficult since 
        \item Formative interviews (first ~3-4 weeks)
            \begin{enumerate}
                \item Might be interesting to curate analysis cases in desktop version
                \item Ask users to interact with mobile version to accomplish same tasks
                \item What interactions did they try to do that worked or didn't work?
                \item What interactions would've helped them be able to answer questions with desktop version
            \end{enumerate}
        \item Interaction pitfalls / taxonomy \\
        Possible interactions: 
            \begin{enumerate}
                \item Gestures (tap, tap+hold, drag, pinch) -- Lots of custom gestures, probably not best
                \item Motion
                \item Portrait vs. landscape
                \item Shake
            \end{enumerate}
        \item Desktop-to-mobile generation system w/ interaction using scoring
        \item Evaluation: How close can we get to desktop version
    \end{enumerate}
}
\jane{Depending on what you're thinking for this part of the approach (point 3), would it make sense to incorporate widgets into the discussion? On the one hand, I think this is different from what you have listed here (which are all forms of user input), whereas widgets are more related to the design decisions of the authors}

\noindent Update interactivity:
\begin{itemize}
    \item \url{https://nyti.ms/3uIKnma} - \jane{This is the network one I was talking about}
    \\ Mobile differences: 
    \begin{enumerate}
        \item Click instead of hover
        \item Remove group labels (e.g., Clinton loyalists)
        \item Stepper through specific people
        \item Display one-to-one relationships instead of many-to-many 
    \end{enumerate}
    
    \item \url{https://n.pr/1IP5XF2} - \jane{Static small multiples -> gif}
    \\ Mobile differences:
    \begin{enumerate}
        \item Merge separate visualization frames / states into automatic animation sequence (i.e., automatic stepper)
        \item No interactivity
    \end{enumerate}
    
    \item \url{https://pudding.cool/2018/12/countries/} - \jane{Tooltip on click not mouseover}
    \\ Mobile differences:
    \begin{enumerate}
        \item Temporary tooltip on tap / click
        \item Removal of linked annotations (desktop interactivity links annotation hover event to corresponding flag)
    \end{enumerate}
    
    \item \url{https://www.nytimes.com/interactive/2019/05/23/opinion/sunday/college-graduation-rates-ranking.html} - \jane{random interaction on mobile with tooltips disabled / dropdown search removed}
    \\ Mobile differences:
    \begin{enumerate}
        \item Tooltips disabled for color-encoded scatter plot
        \item Visualization views separated into multiple states (combined with text scrolling on desktop)
        \item Dropdown search removed
    \end{enumerate}
    
\end{itemize}

\noindent Disable interactivity:
\begin{itemize}
    \item \url{https://www.nationalgeographic.com/what-the-world-eats/} - \jane{This example has an interactivity ``warning label'' on mobile: ``Visit this site on your desktop browser or tablet device to explore the full interactive version...''}
    \\ Mobile differences:
    \begin{enumerate}
        \item Click on pie slices instead of hover (desktop)
        \item ``Full interactivity'' desktop version provides country-level aggregation previews
    \end{enumerate}
    
    \item \url{https://nyti.ms/2nCtGXG}
    \\ Mobile differences:
    \begin{enumerate}
        \item Removed all hover interactions
        \item Removed filter dropdown
    \end{enumerate}
    
    \item \url{https://www.nytimes.com/interactive/2019/01/26/opinion/sunday/paths-to-congress.html} - \jane{Interesting because the mobile version adds multiple static charts in place of the interactive design (but not all of it)}
    \\ Mobile differences:
    \begin{enumerate}
        \item Removed all hover and dropdown interactions (used for senator filtering)
    \end{enumerate}
    
    \item \url{https://projects.fivethirtyeight.com/2018-march-madness-predictions/} - \jane{Remove option to change between bracket/table}
    \\ Mobile differences:
    \begin{enumerate}
        \item Bracket visualization with hovering removed
    \end{enumerate}
        
    \item \url{https://www.nationalgeographic.com/foodfeatures/diet-similarity/} - \jane{Remove interaction and only shown end result}
    \\ Mobile differences:
    \begin{enumerate}
        \item Time slider removed
        \item Hover path tooltips removed
    \end{enumerate}
    
\end{itemize}


==> sections/3-designguidelines.tex <==
\section{Design Guidelines}
%%
%% Note: Comment in one of the following labels for the section to keep track of progress
%%
    %\complete
    %\feedbackProvided
    %\readyForFeedback
    %\underRevision
    \incomplete
%%
%% Note: Add the content for the section directly after this comment
%%
\subsection{Common Issues \& Points of Reflection}
Selection\\
Tailored interactions (for specific visualization) \\
Complex gestures \\
Complex modalities (limiting flexibility / accessibility) \\
Fat-finger \\
Maintain context / context switching (e.g., having to zoom back and forth) \\
Not interrupt analysis / exploratory workflow \\
Simple tasks may be difficult \\
Exploratory ''workbooks'' \\
Limited screen size (need better interactions) \\



\subsection{Initial Guidelines}
Mobile devices are more often used\\
-- Portable\\
-- Accessible\\

Want interactions to be: \\
(1) Easy to use\\
    -- Use existing touch / motion gestures people are familiar with and similar metaphors\\
(2) Responsive\\
(3) Flexible (?)\\
-- Used for different visualizations\\
-- Adapt interactions to scale, encoding types\\
-- Support wide range of exploratory tasks\\
(4) Efficient\\
-- Mobile devices are good for ''brevity''\\
-- Get quick overview\\
-- Do simple select, inspect\\
-- Want interactions that can do these tasks pretty seamlessly\\


==> sections/6-evaluationusecases.tex <==
\section{Evaluation: Case Studies}
%%
%% Note: Comment in one of the following labels for the section to keep track of progress
%%
    %\complete
    %\feedbackProvided
    %\readyForFeedback
    %\underRevision
    \incomplete
%%
%% Note: Add the content for the section directly after this comment
%%


==> sections/7-evaluationuserstudy.tex <==
\section{Evaluation: User Study}
%%
%% Note: Comment in one of the following labels for the section to keep track of progress
%%
    %\complete
    %\feedbackProvided
    %\readyForFeedback
    %\underRevision
    \incomplete
%%
%% Note: Add the content for the section directly after this comment
%%

\subsection{Methods}

\subsection{Results}

